Bayesian learning of weakly structural Markov graph laws using sequential Monte Carlo methods

We present a sequential sampling methodology for weakly structural Markov laws, arising naturally in a Bayesian structure learning context for decomposable graphical models. As a key component of our suggested approach, we show that the problem of graph estimation, which in general lacks natural sequential interpretation, can be recast into a sequential setting by proposing a recursive Feynman-Kac model that generates a flow of junction tree distributions over a space of increasing dimensions. We focus on particle McMC methods to provide samples on this space, in particular on particle Gibbs (PG), as it allows for generating McMC chains with global moves on an underlying space of decomposable graphs. To further improve the PG mixing properties, we incorporate a systematic refreshment step implemented through direct sampling from a backward kernel. The theoretical properties of the algorithm are investigated, showing that the proposed refreshment step improves the performance in terms of asymptotic variance of the estimated distribution. The suggested sampling methodology is illustrated through a collection of numerical examples demonstrating high accuracy in Bayesian graph structure learning in both discrete and continuous graphical models.

==> __latexindent_temp.tex <==
% -*- root: opr_2016_main.tex -*-
\section{}\label{sec:appendix}

\subsection{Graph theory}\label{sec:graphtheory}
Given a set $V = \{a_1, \ldots, a_p\}$ of $p \in \nsetpos$ distinct elements,
an \emph{undirected graph} $\graph$ with \emph{nodes} $\graphnodeset$
is specified by a set of \emph{edges} $\graphedgeset \subseteq \graphnodeset
\times \graphnodeset$, and we write $\graph = (\graphnodeset ,\graphedgeset)$.
In addition, we say that $\graph' = (\graphnodeset', \graphedgeset')$ is a
\emph{subgraph} of $\graph$ if $\graphnodeset' \subseteq \graphnodeset$
and $\graphedgeset' \subset \graphedgeset$. For any pair $(a, b)$ of nodes
in $\graph$, a \emph{path} from $a$ to $b$, denoted by $a \sim b$, is a
sequence $\{ a_{n_k} \}_{k = 1}^{\ell + 1}$, with $\ell \in \intvect{1}{p - 1}$, of
distinct nodes such that $a_{n_1} = a$, $a_{n_{\ell + 1}} = b$, and
$(a_{n_k}, a_{n_{k + 1}}) \in \graphedgeset$ for all $k \in \intvect{1}{\ell}$.
Here $\ell$ is called the \emph{length} of the path.  A graph is called a
\emph{tree} if there is a unique path between any pair of nodes.
A graph is \emph{connected} when there is a path between every pair
of nodes, and a \emph{subtree} is a connected subgraph of a tree.
Let $\graph =  (\graphnodeset ,\graphedgeset)$ be a graph and $A$, $B$,
and $S$ subsets of $\graphnodeset$; then $S$ is said to \emph{separate}
$A$ from $B$ if for all $a \in A$ and $b \in B$, every path $a \sim b$ intersects $S$.
This is denoted by $A \perp_{\graph} B \mid S$. A graph is \emph{complete}
if $\graphedgeset = \graphnodeset \times \graphnodeset$. Let $\graphnodeset'
\subseteq \graphnodeset$; then the \emph{induced subgraph}
$\graph {[\graphnodeset']} = (\graphnodeset', \graphedgeset')$ is the subgraph
of $\graph$ with nodes $\graphnodeset'$ and edges $\graphedgeset'$ given
by the subset of edges in $\graphedgeset$ having both endpoints in $\graphnodeset'$.
We write $\graph' = (\graphnodeset', \graphedgeset') \leq \graph = (\graphnodeset,
\graphedgeset)$ to indicate that $\graph' = \graph {[\graphnodeset']}$. A subset
$W \subseteq \graphnodeset$ is a \emph{complete set} if it induces a complete
subgraph. A complete subgraph is called a \emph{clique} if it is not an induced
subgraph of any other complete subgraph. We denote by $\clset{G}$ the family
of cliques formed by a graph $G$.\footnote{We use calligraphy
uppercase to denote families of graphs, or, more generally, families of sets
(as a graph is, given the nodes, specified through the edge set). Consequently,
calligraphy uppercase will also used to denote $\sigma$-fields.} A triple $(A, B, S)$
of disjoint subsets of $\graphnodeset$ is a \emph{decomposition} of
$\graph = (\graphnodeset, \graphedgeset)$ if $A \cup B \cup S=\graphnodeset$,
$A \neq \varnothing$, $B \neq \varnothing$, $S$ is complete, and it holds that
$A \perp_{\graph} B \mid S$.



\subsection{Proofs and lemmas}
\label{sec:proofslemmas}
The following lemma, proved in a slightly different form in \cite{doi:10.1198/jcgs.2009.07129}, establishes that each extension
\eqref{def:extended:tree:meas} has the correct marginal
w.r.t. the graph, i.e., that $\graphtarg[\A]$ is the distribution
of $\trgr(\tau)$ when $\tau \sim \trtarg[\A]$.
\begin{lemma} \label{lemma:preservation:marginal}
	For all $\A \subseteq \graphnodeset$ and $h \in \mf{\graphfd}$,
	$$
		\E_{\trtarg[\A]} \left[ h \circ \trgr(\tau) \right] = \graphtarg[\A] h,
	$$
	where $\trtarg[\A]$ is defined in \eqref{def:extended:tree:meas}.
\end{lemma}
\begin{proof}
%See Appendix~\ref{lemma:preservation:marginal:proof}.
%\end{proof}
%\begin{proof}[Proof of Lemma~\ref{lemma:preservation:marginal}]
	\label{lemma:preservation:marginal:proof}
	Since
	\begin{multline*}
		\untrtarg[\A] \1_{\trsp[\A]}
		= \sum_{\tree \in \trsp[\A]} \untrtarg[\A](\tree)
		= \sum_{\graph \in \graphsp[\A]} \sum_{\tree \in \grtr(\graph)}
		\frac{\ungraphtarg[\A] \circ \trgr(\tree)}{\mu \circ \trgr(\tree)} \\
		= \sum_{\graph \in \graphsp[\A]} \mu(\graph)
		\frac{\ungraphtarg[\A](\graph)}{\mu(\graph)}
		= \ungraphtarg[\A] \1_{\graphsp[\A]},
	\end{multline*}
	it holds that
	\begin{equation} \label{eq:trtarg:alt:representation}
		\trtarg[\A](\rmd \tree) =
		\frac{\graphtarg[\A] \circ \trgr(\tree)}
		{\mu \circ \trgr(\tree)} \, \cm{\rmd \tree}.
	\end{equation}
	Now, let $h \in \mf{\graphfd[\A]}$; then by a similar computation,
	\begin{multline*}
		\E_{\trtarg[\A]} \left[ h \circ \trgr(\tree) \right]
		= \sum_{\graph \in \graphsp[\A]} \sum_{\tree \in \grtr(\graph)}
		h \circ \trgr(\tree) \frac{\graphtarg[\A] \circ \trgr(\tree)}
		{\mu \circ \trgr(\tree)} \\
		= \sum_{\graph \in \graphsp[\A]} \mu(\graph) h(\graph)
		\frac{\graphtarg[\A](\graph)}{\mu(\graph)} = \graphtarg[\A] h,
	\end{multline*}
	which completes the proof.
\end{proof}


\begin{proof}[Proof of Theorem \ref{thm:asymvar}]
\label{proof:asymvar}
	First, as established in \cite[Proposition~8]{chopin:singh:2015}, the standard
	PG kernel $\PG{p}$ is $\targ{1:p}$-reversible. As mentioned above, the kernel
	$\G{p}$ is straightforwardly $\targ{1:p}$-reversible as a standard Gibbs substep.
	Moreover, for all $\x{1:p} \in \xsp{1:p}$, $\G{p}(\x{1:p}, \xsp{1:p - 1} \times \{\x{p} \}) = 1$
	and $\G{p}$ dominates trivially the Dirac mass on the \emph{off-diagonal},
	in the sense that for all $A \in \xfd{1:p}$ and $\x{1:p} \in \xsp{1:p}$,
	$\G{p}(\x{1:p}, A \setminus \x{1:p}) \geq \delta_{\x{1:p}}(A \setminus \x{1:p}) = 0$.
	The assumptions of \cite[Lemma~18]{maire:douc:olsson:2014} are thus fulfilled,
	and the proof is concluded through application of the latter.
\end{proof}




==> commands.tex <==
\newtheorem{theorem}{Theorem}

\newaliascnt{definition}{theorem}
\newtheorem{definition}[definition]{Definition}
\aliascntresetthe{definition}

\newaliascnt{lemma}{theorem}
\newtheorem{lemma}[lemma]{Lemma}
\aliascntresetthe{lemma}
\crefname{lemma}{lemma}{lemmas}
\Crefname{Lemma}{Lemma}{Lemmas}


% Commands IN ALPHABETIC ORDER

\newcommand{\gen}[1]{J_{#1}}
\newcommandx{\bk}[2][1=]{
\ifthenelse{\equal{#1}{}}
{\kernel{R}_{#2}}
{\kernel{R}_{#2} \langle #1 \rangle}
}
\newcommand{\bmf}[1]{\mathbb{F}_{\mathrm{b}}(#1)}
%\newcommand{\cloud}[1]{\boldsymbol{\tau}_{#1}^\N}
\def\bs#1{\mbox{$\boldsymbol#1$}}
\newcommand{\card}{\operatorname{Card}}
\newcommand{\cloud}[1]{\tau_{#1}^{1:\N}}
\newcommand{\cm}[1]{|#1|}
\newcommandx{\comb}[2][1=]{
\ifthenelse{\equal{#1}{}}
{s_{#2}}
{s_{#1 \mid #2}}
}
\newcommand{\combkernel}[1]{\kernel{\Sigma}_{#1}}
\newcommand{\combkernelpath}[1]{\bar{\kernel{\Sigma}}_{#1}}
\newcommand{\combmeas}[1]{\sigma_{#1}}
\newcommand{\combpart}[2]{\varsigma_{#1}^{#2}}
\newcommand{\combsp}[1]{\spc{S}_{#1}}
\newcommand{\disc}{\mathsf{Pr}}
\newcommand{\dens}{f}
\newcommand{\E}{\mathbb{E}}
\newcommand{\epart}[2]{\xi_{#1}^{#2}}
\newcommand{\eqdef}{\vcentcolon=}
\newcommand{\G}[1]{\kernel{G}_{#1}}
\newcommandx{\graph}[1][1=]{\ifthenelse{\equal{#1}{}}{G}{G_{#1}}}
\newcommandx{\graphedgeset}[1][1=]{\ifthenelse{\equal{#1}{}}{E}{E_{\mathsmaller{#1}}}}
\newcommandx{\graphfd}[1][1=]{\ifthenelse{\equal{#1}{}}{\mathcal{G}}{\mathcal{G}_{#1}}}
\newcommandx{\graphnodeset}[1][1=]{\ifthenelse{\equal{#1}{}}{V}{V_{\mathsmaller{#1}}}}
%\newcommand{\gr}[1]{G_{#1}}
\newcommandx{\graphsp}[1][1=]{\ifthenelse{\equal{#1}{}}{\mathsf{G}}{\mathsf{G}_{#1}}}
\newcommandx{\graphtarg}[1][1=]{\ifthenelse{\equal{#1}{}}{\graphtargletter^\star}{\graphtargletter^\star \langle #1 \rangle}}
\newcommand{\graphtargletter}{\eta}
%\newcommand{\graphtarg}[1]{\ifthenelse{\equal{#1}{}}{\pi}{\pi_{#1}}}
\newcommand{\grtr}{t}
\newcommand{\hypdircount}{\vartheta}
\newcommand{\ind}[2]{I_{#1}^{#2}}
%\newcommand{\indset}{\mathsf{S}}
\newcommand{\intvect}[2]{\llbracket #1, #2 \rrbracket}
\newcommand{\jimmy}[1]{\todo[color=blue!20]{{\bf Jimmy:} #1}}
\newcommandx{\jtnode}[1][1=]{\ifthenelse{\equal{#1}{}}{c}{c_{#1}}}
\newcommand{\jtorder}{k}
\newcommand{\kernel}[1]{\mathbf{#1}}
\newcommand{\meas}[1]{\mathbb{M}(#1)}
\newcommand{\mf}[1]{\mathbb{F}(#1)}
\newcommand{\N}{N}
\newcommandx{\nckernel}[2][1=]{
\ifthenelse{\equal{#1}{}}
{\boldsymbol{\Gamma}_{#2}}
{\boldsymbol{\Gamma}_{#2} \langle #1 \rangle}
}
\newcommand{\normconst}{I}
\newcommand{\nset}{\mathbb{N}}
\newcommand{\nsetpos}{\mathbb{N}^*}
%\newcommand{\ntrees}[2]{\mu_{#1}(#2)}
\newcommand{\ntrees}[2]{\mu(#2)}
\newcommand{\1}{\mathbbm{1}}
\newcommand{\p}{p}
\newcommand{\param}{\theta}
\newcommand{\paramref}{\lambda}
\newcommand{\paramsp}{\Theta}
\newcommand{\paramfd}{\mathcal{P}}
\newcommandx{\partarg}[2][1=]{
    \ifthenelse{\equal{#1}{}}
    {\eta^{\N}_{#2}}
    {\eta_{#2}^{\ast, \N}}
}
\newcommandx{\partinit}[1][1=]{
       \ifthenelse{\equal{#1}{}}
       {\kappa}
       {\kappa^\ast \langle #1 \rangle}
}
\newcommandx{\perm}[2][2=]{
\ifthenelse{\equal{#2}{}}
{s_{#1}}
{s_{#1}(#2)}
}
%\newcommandx{\perm}[2][2=]{
%\ifthenelse{\equal{#2}{}}
%{s(#1)}
%{s_{#1}(#2)}
%}
\newcommand{\PG}[1]{\kernel{P}_{#1}^\N}
\newcommand{\pMCMCprop}[1]{\rho_{#1}^\N}
\newcommand{\pMCMCtarg}[1]{\pi_{#1}^\N}
\newcommand{\posterior}{\pi}
\newcommand{\potset}{\boldsymbol{\wp}}
\newcommand{\prior}{\pi}
\newcommand{\precmat}{\theta}

\newcommand{\priorkernel}{\boldsymbol{\Pi}}
%\newcommand{\priorkernel}{\mathbf{T}}
\newcommand{\probmeas}[1]{\mathbb{M}_1(#1)}
\newcommandx{\prop}[2][1=]{
\ifthenelse{\equal{#1}{}}
{\kernel{\propletter}_{#2}}
{\kernel{\propletter}_{#2}^\ast \langle #1 \rangle}
}
\newcommand{\propletter}{K}
\newcommandx{\proppath}[2][1=]{
\ifthenelse{\equal{#1}{}}
{\bar{\kernel{\propletter}}_{#2}}
{\bar{\kernel{\propletter}}_{#2} \langle #1 \rangle}
}

\newcommand{\randind}[1]{\iota}%_{#1}}
\newcommand{\randperm}[1]{\varsigma_{#1}}
\newcommand{\refm}{\nu}
\newcommand{\retrosupp}[1]{\mathsf{S}_{#1}}
\newcommand{\rset}{\mathbb{R}}
\newcommand{\rsetnonneg}{\mathbb{R}_+}
\newcommand{\rvalfun}[1]{\mathbb{F}(#1)}
%\newcommand{\targex}
%\newcommandx{\targ}[2][1=]{
%    \ifthenelse{\equal{#1}{}}
%    {\eta_{#2}}
%    {\eta_{#2}^\ast}
%}
%\newcommand{\rmd}{\operatorname{d}}
\newcommand{\rmd}{d}
\newcommandx{\SMCdist}[2][1=]{
\ifthenelse{\equal{#1}{}}
{\varrho_{#2}^\N}
{\varrho_{#2}^\N \langle #1 \rangle}
}
\newcommand{\spc}[1]{\mathsf{#1}}

\newcommand{\supp}{\operatorname{Supp}}
%\newcommand{\sym}{\operatorname{Sym}}
\newcommand{\sym}[1]{\Sigma_{#1}}
\newcommand{\symmeas}[1]{\sigma_{#1}}
\newcommandx{\targ}[3][1=, 3=]{
   \ifthenelse{\equal{#3}{}}
   {
       \ifthenelse{\equal{#1}{}}
       {\eta_{#2}}
       {\eta^\ast \langle #2 \rangle}
%       {\eta_{#2}}
%       {\eta_{#2}^\ast}
   }
   {
       \ifthenelse{\equal{#1}{}}
       {\eta_{#2} \langle #3 \rangle}
       {\eta_{#2}^\ast \langle #3 \rangle}
   }
}
\newcommandx{\targMCMC}[3][1=]{
\ifthenelse{\equal{#1}{}}
{\eta_{#2}^{\N, #3}}
{\eta^* \langle #2 \rangle^{\N, #3}}
}
\newcommand{\targpath}[1]{\bar{\eta}_{#1}}
\newcommand{\tbw}{(To be written.)}
\newcommandx{\tree}[1][1=]{\ifthenelse{\equal{#1}{}}{T}{T_{\mathsmaller{#1}}}}
\newcommandx{\treerv}[1][1=]{\ifthenelse{\equal{#1}{}}{\mathcal T}{\mathcal T_{#1}}}
\newcommandx{\tr}[2][2=]{
\ifthenelse{\equal{#2}{}}
{\tilde{x}_{#1}}
{\tilde{x}_{#1}^{#2}}
}
\newcommand{\trexfd}[1]{\mathcal{X}_{#1}}
\newcommand{\trexsp}[1]{\mathsf{X}_{#1}}
\newcommand{\treefd}[1]{\tilde{\mathcal{X}}_{#1}}
\newcommand{\treesp}[1]{\tilde{\mathsf{X}}_{#1}}
\newcommandx{\trex}[2][2=]{
\ifthenelse{\equal{#2}{}}
{x_{#1}}
{x_{#1}^{#2}}
}

\newcommandx{\trfd}[1][1=]{\ifthenelse{\equal{#1}{}}{\mathcal{T}}{\mathcal{T}_{#1}}}
\newcommand{\trgr}{g}
\newcommandx{\trsp}[1][1=]{\ifthenelse{\equal{#1}{}}{\mathsf{T}}{\mathsf{T}_{#1}}}
\newcommandx{\trtarg}[1][1=]{\ifthenelse{\equal{#1}{}}{\eta^\ast}{\eta^\ast \langle #1 \rangle}}
\newcommand{\ukpath}[1]{\bar{\kernel{Q}}_{#1}}
\newcommandx{\uk}[2][1=]{
\ifthenelse{\equal{#1}{}}
{\kernel{Q}_{#2}}
{\kernel{Q}_{#2} \langle #1 \rangle}
}
\newcommandx{\ungraphtarg}[1][1=]{\ifthenelse{\equal{#1}{}}{\gamma^\star}{\gamma^\star \langle #1 \rangle}}
\newcommandx{\untarg}[3][1=, 3=]{
   \ifthenelse{\equal{#3}{}}
   {
       \ifthenelse{\equal{#1}{}}
%       {\gamma_{#2}}
%       {\gamma_{#2}^\ast}
       {\gamma_{#2}}
       {\gamma^\ast \langle #2 \rangle}
   }
   {
       \ifthenelse{\equal{#1}{}}
       {\gamma_{#2} \langle #3 \rangle}
       {\gamma_{#2}^\ast \langle #3 \rangle}
   }
}
\newcommandx{\untrtarg}[1][1=]{\ifthenelse{\equal{#1}{}}{\gamma^\ast}{\gamma^\ast \langle #1 \rangle}}
\newcommand{\untargpath}[1]{\bar{\gamma}_{#1}}
\newcommandx{\unpartarg}[2][1=]{
    \ifthenelse{\equal{#1}{}}
    {\gamma_{#2}^\N}
    {\gamma_{#2}^\N  \langle #1 \rangle}
}

\newcommand{\wgt}[2]{\omega_{#1}^{#2}}
\newcommandx{\wgtfunc}[2][1=]{
\ifthenelse{\equal{#1}{}}
{w_{#2}}
{w_{#2} \langle #1 \rangle}
}
\newcommand{\wgtsum}[1]{\Omega_{#1}^\N}
\newcommandx{\x}[2][2=]{
\ifthenelse{\equal{#2}{}}
{x_{#1}}
{x_{#1}^{#2}}
}
\newcommandx{\X}[2][2=]{
\ifthenelse{\equal{#2}{}}
{X_{#1}}
{X_{#1}^{#2}}
}
\newcommandx{\xt}[2][2=]{
\ifthenelse{\equal{#2}{}}
{\tilde{x}_{#1}}
{\tilde{x}_{#1}^{#2}}
}
\newcommandx{\Xt}[2][2=]{
\ifthenelse{\equal{#2}{}}
{\tilde{X}_{#1}}
{\tilde{X}_{#1}^{#2}}
}

\newcommand{\xfd}[1]{\mathcal{X}_{#1}}
\newcommand{\xsp}[1]{\mathsf{X}_{#1}}
\newcommand{\xtfd}[1]{\tilde{\mathcal{X}}_{#1}}
\newcommand{\xtsp}[1]{\tilde{\mathsf{X}}_{#1}}
\newcommandx{\y}[1][1=]{\ifthenelse{\equal{#1}{}}{y}{y_{#1}}}
\newcommandx{\Y}[1][1=]{\ifthenelse{\equal{#1}{}}{Y}{Y_{#1}}}
\newcommandx{\ysp}[1][1=]{\ifthenelse{\equal{#1}{}}{\mathsf{Y}}{\mathsf{Y}_{#1}}}
\newcommandx{\yfd}[1][1=]{\ifthenelse{\equal{#1}{}}{\mathcal{Y}}{\mathcal{Y}_{#1}}}
\newcommandx{\z}[2][2=]{
\ifthenelse{\equal{#2}{}}
{z_{#1}}
{z_{#1}^{#2}}
}
\newcommandx{\Z}[2][2=]{
\ifthenelse{\equal{#2}{}}
{Z_{#1}}
{Z_{#1}^{#2}}
}

\newcommand{\zfd}[1]{\mathcal{Z}_{#1}}
\newcommand{\zpart}[2]{\zeta_{#1}^{#2}}
\newcommand{\zsp}[1]{\mathsf{Z}_{#1}}




==> opr_2016_problem_statement.tex <==
% -*- root: opr_2016_main.tex -*-
From now on, let $\graphnodeset$ be a fixed set of $p \in \nsetpos$
distinct vertices. Without loss of generality, we let $\graphnodeset = \intvect{1}{p}$.
For $\subnodeset \subseteq \graphnodeset$, we denote by $\graphsp[\subnodeset]$
the space of decomposable graphs with vertices $\subnodeset$, i.e.,
$\graphsp[\subnodeset] \eqdef \{(\subnodeset, E) : E \subseteq
\subnodeset \times \subnodeset \}$. In particular, set $\graphsp
\eqdef \graphsp[V]$. In addition, let $\allgr \eqdef \cup_{\subnodeset \subseteq \graphnodeset}
\graphsp[\subnodeset]$ be the space of all decomposable graphs with vertices
given by $\graphnodeset$ or some subset of the same.

\begin{definition} \label{def:CFS}
A positive function $\graphmap$ on $\allgr$ is said to satisfy the
\emph{clique-separator factorisation} (\CSF) if for all $G \in \allgr$,
$$
	\graphmap(G) = \frac{\prod_{\cl \in \clset{G}} \graphmap(\graph[\cl])}
	{\prod_{S \in \sepset{G}} \graphmap(\graph[S])}.
$$
\end{definition}

For some given function $\graphmap$ satisfying the \CSF, the aim
of this paper is to develop a strategy for sampling from the family of so called \emph{weakly structural Markov} distributions \citep{green2017structural}, which assuming full support on $\graphsp$, are characterised as
\begin{equation} \label{eq:graph:target}
	\graphtarg(\rmd \graph) = \frac{\ungraphtarg(\rmd \graph)}
	{\ungraphtarg \1_{\graphsp}}
\end{equation}
on $\probmeas{\graphsp}$, where
$$
	\ungraphtarg(\rmd \graph) \eqdef
	\graphmap |_{\graphsp} (\graph) \, \cm{\rmd \graph},
$$
with $\graphmap |_{\graphsp}$ denoting the restriction of $\graphmap$
to $\graphsp$ and $\cm{\rmd \graph}$ the counting measure on $\graphsp$.
The normalising constant $\ungraphtarg \1_{\graphsp} =
\sum_{\graph \in \graphsp} \ungraphtarg(\graph)$ will be considered
as intractable, as computing the same requires the summation of over
the whole space $\graphsp$, which is impractical as the cardinality of
$\graphsp$ is immense already for moderate $p$.

